Pushing the Boundaries of Tractable Multiperspective Reasoning: A Deduction Calculus for Standpoint EL+

Standpoint EL is a multi-modal extension of the popular description logic EL that allows for the integrated representation of domain knowledge relative to diverse standpoints or perspectives. Advantageously, its satisfiability problem has recently been shown to be in PTime, making it a promising framework for large-scale knowledge integration. In this paper, we show that we can further push the expressivity of this formalism, arriving at an extended logic, called Standpoint EL+, which allows for axiom negation, role chain axioms, self-loops, and other features, while maintaining tractability. This is achieved by designing a satisfiability-checking deduction calculus, which at the same time addresses the need for practical algorithms. We demonstrate the feasibility of our calculus by presenting a prototypical Datalog implementation of its deduction rules.

==> mymacros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                    ** mymacros.tex **                     %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\usepackage{comment}
%\usepackage{ifpdf}

% hs macros
\newcommand{\email}[1]{\href{mailto:#1}{#1}}
% math & logic
\newcommand{\set}[1]{\left\{#1\right\}}
\newcommand{\guard}{\mathrel{\left.\middle\vert\right.}}
\newcommand{\card}[1]{\left\vert#1\right\vert}
\newcommand{\size}[1]{\left\Vert#1\right\Vert}
\newcommand{\iffdef}{\mathrel{{\iff\!}_{\mbox{\em\tiny def}}}}
\newcommand{\bigland}{\bigwedge}
\newcommand{\biglor}{\bigvee}
\newcommand{\limplies}{\rightarrow}
\newcommand{\Trans}{\mathrm{Trans}}
\newcommand{\trans}{\mathrm{trans}}
\newcommand{\svec}[1]{\vec{#1}\,}
\newcommand{\pick}[1]{\mathsf{pick}\!\left(#1\right)}
% paper-specific special symbols
\newcommand{\Sub}{\mathit{Sub}}
\newcommand{\M}{\mathcal{M}}
\renewcommand{\S}{\mathcal{S}}
\newcommand{\PV}[1]{\mathcal{P}_{#1}}
\newcommand{\Pphi}{\PV{\phi}}
\newcommand{\preq}{\simeq}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  END END END         (of mymacros.tex)      END END END   %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> sections/calculus.tex <==
\paragraph{Deduction Rules}{$\left.\right.$}
\\

\newcommand{\dedsr}[3]{$\begin{array}{@{\,}c@{\,}}{#1}\\[-2.2ex]\\\hline\\[-2.2ex]{#2}\end{array}{\ \ (#3)}$}

%Sharpening derivations
%\medskip
%
%\dedsr{{}} {\st \preceq *}
%\qquad
%\dedsr{{\st \preceq \sp \quad \sp \preceq \spp}} {\st \preceq \spp}
%
%\medskip

\def\axA{1\xspace}
\def\axB{2\xspace}
\def\axC{3\xspace}
\def\axD{4\xspace}
\def\hierA{5\xspace}
\def\hierB{6\xspace}
\def\inhierA{7\xspace}
\def\inhierB{8\xspace}
\def\inhierC{9\xspace}
\def\inhierD{10\xspace}
    \def\inhierE{40\xspace}
    \def\inhierF{44\xspace}
    \def\inhierG{42\xspace}
    \def\locB{43\xspace}
\def\subA{11\xspace}
\def\subB{12\xspace}
\def\subC{13\xspace}
\def\subD{14\xspace}
\def\flatA{15\xspace}
\def\flatB{16\xspace}
\def\flatC{17\xspace}
\def\flatD{18\xspace}
\def\con{19\xspace}
\def\exA{20\xspace}
\def\exB{21\xspace}
\def\exC{22\xspace}
\def\loc{23\xspace}
\def\retA{24\xspace}
\def\retB{25\xspace}
\def\retC{26\xspace}
    \def\abAA{39\xspace}
\def\abA{27\xspace}
\def\abB{28\xspace}
\def\abC{29\xspace}
\def\abeA{30\xspace}
\def\abeB{31\xspace}
\def\abr{32\xspace}
\def\selfA{33\xspace}
\def\selfB{34\xspace}
\def\selfC{35\xspace}
\def\selfD{36\xspace}
\def\selfE{37\xspace}
\def\selfF{38\xspace}
    \def\fixA{41\xspace}

Axioms (for all $\st\in \Stands$ and concept names $C$)

\dedsr{{}} {\st \preceq *}{\axA}
\qquad
\dedsr{{}} {\st \preceq \st}{NEW}
\qquad
\dedsr{{}} {\top \sqsubseteq \standball [ C \Rightarrow C ] }{\axB}
\qquad
\dedsr{{}} {\top \sqsubseteq \standball	[ C \Rightarrow \top ] }{\axC}
\qquad
\dedsr{{}} {\standball[R \sqsubseteq R]}{\axD}
\bigskip

Standpoint hierarchy rules

\dedsr{{\st \preceq \sp \quad \sp \preceq \spp}} {\st \preceq \spp}{\hierA}
\qquad
\dedsr{{\st \preceq \st_1 \quad \st \preceq \st_2 \quad \st_1 \cap \st_2 \preceq \sp}} {\st \preceq \sp}{\hierB}

Inheritance along the standpoint hierarchy

\medskip

\dedsr{	\standb{s'} [R \sqsubseteq R'] \quad \st \preceq \sp } {\standb{s} [R \sqsubseteq R'] }{\inhierA}
\qquad
\dedsr{	C \sqsubseteq \standb{s'} [D \Rightarrow E] \quad \st \preceq \sp } {C \sqsubseteq \standb{s} [D \Rightarrow E] }{\inhierB}

\medskip

\dedsr{ \standb{s'} [C \sqsubseteq \exists R.D] \quad \st \preceq \sp } {\standb{s} [C \sqsubseteq \exists R.D] }{\inhierC}\qquad
\dedsr{ \standb{s'} [\exists R.D \sqsubseteq C] \quad \st \preceq \sp } {\standb{s} [\exists R.D \sqsubseteq C] }{\inhierD}
\qquad
\dedsr{	\standb{s'} [C_1 \sqcap C_2 \sqsubseteq  D]  \quad \st \preceq \sp } { \standb{s} [C_1 \sqcap C_2 \sqsubseteq  D]  }{\inhierE}

\bigskip

Inferences among subclass statements

\medskip

\dedsr{ B \sqsubseteq 	\standb{s}	[C \Rightarrow  D] \quad B \sqsubseteq  \standb{s}	[D \Rightarrow E] } { B \sqsubseteq  \standb{s}	[C \Rightarrow E] }{\subA}
\qquad
\dedsr{	\top \sqsubseteq \standball [ B \Rightarrow C ] \quad C \sqsubseteq \standb{s} [D \Rightarrow E ] } {  B \sqsubseteq \standb{s} [ D \Rightarrow E ] }{\subB}{maybe not needed}

\medskip

\dedsr{	\top \sqsubseteq \standball [ C \Rightarrow D ] \quad D \sqsubseteq \standd{s} E} { C \sqsubseteq \standd{s} E}{\subC}maybe not needed
\qquad
\dedsr{	 C \sqsubseteq  \standd{s} D  \quad C \sqsubseteq \standb{s} [ D \Rightarrow  E ] } { C \sqsubseteq \standd{s} E  }{\subD}


\bigskip

Flattening of modalities

\medskip

\dedsr{	 C \sqsubseteq  \standb{s'} [\top \Rightarrow D] \quad  D \sqsubseteq \standb{s} [E \Rightarrow F]  } { C \sqsubseteq \standb{s} [E \Rightarrow F] }{\flatA}
\qquad
\dedsr{	 C \sqsubseteq  \standb{s'} [\top \Rightarrow D]  \quad  D \sqsubseteq \standd{s} E  } {  C \sqsubseteq \standd{s} E  }{\flatB}


\medskip

\dedsr{ C \sqsubseteq  \standd{s'} D  \quad D \sqsubseteq \standb{s} [E \Rightarrow F] } { C \sqsubseteq \standb{s} [E \Rightarrow F] }{\flatC}
\qquad
\dedsr{ C \sqsubseteq  \standd{s'} D \quad D \sqsubseteq \standd{s} E } { C \sqsubseteq \standd{s} E }{\flatD}

\bigskip

Inference involving conjunction

\medskip


\dedsr{	B \sqsubseteq \standb{s} [ C \Rightarrow  C_1 ] \quad B \sqsubseteq \standb{s} [ C \Rightarrow  C_2 ] \quad \standb{s} [C_1 \sqcap C_2 \sqsubseteq  D] } { B \sqsubseteq \standb{s} [C \Rightarrow  D] }{\con}

%\medskip
%
%\dedsr{ \standball [ C \sqsubseteq  \standb{s} C_1 ] \quad C \sqsubseteq  \standd{s} C_2 \quad C_1 \sqcap C_2 \equiv  D } {C \sqsubseteq  \standd{s} D } \qquad (??? plus symmetric version) MIRACULOUSLY NOT NEEDED

\bigskip

Inferences involving existential quantifiers

\medskip

\dedsr{ \standb{s} [C \sqsubseteq \exists R. D] \quad \top \sqsubseteq \standb{s} [ D \Rightarrow E ] \quad \standb{s} [ R \sqsubseteq R' ]}
{ \standb{s} [C \sqsubseteq \exists R'. E] }{\exA}
%{\color{teal} NEW VERSION OF PREVIOUS (NEEDED??):\\ 
%\dedsr{ C \sqsubseteq \exists R. D \quad \top \sqsubseteq \standball [ D \Rightarrow E ] \quad  R \sqsubseteq R' }
%{ C \sqsubseteq \exists R'. E }{\exA}
%}
\qquad
\dedsr{ \standb{s} [C \sqsubseteq \exists R. D] \quad \standb{s} [\exists R. D \sqsubseteq F] } {\top \sqsubseteq \standb{s} [C \Rightarrow F] }{\exB}
%{\\ \color{teal} NEW VERSION OF PREVIOUS (NEEDED!!):\\ 
%\dedsr{ C \sqsubseteq \exists R. D \quad \top \sqsubseteq \standbs [ D \Rightarrow E ] \quad \exists R. E \sqsubseteq F } {\top %\sqsubseteq \standb{s} [C \Rightarrow F] }{\exB}
%}

\medskip
\dedsr{ \standb{s} [C \sqsubseteq \exists R_1. D] \quad \standb{s} [D \sqsubseteq \exists R_2.E] \quad  \standb{s}	[ R_1 \circ R_2  \sqsubseteq R' ]}{ \standb{s} [C \sqsubseteq \exists R'. E] }{\exC}




\bigskip

``Localisation'' of subsumptions

\medskip

\qquad
\dedsr{	C \sqsubseteq \standb{s} [ \top \Rightarrow D]  } {\top \sqsubseteq \standb{s}	[C \Rightarrow D] }{\loc}

\bigskip

``Retraction'' of $\bot$ inferences

\medskip

\dedsr{ \standb{s} [C \sqsubseteq \exists r. \bot ] } {\top \sqsubseteq \standb{s} [C \Rightarrow \bot] }{\retA}
\qquad
\dedsr{	 C \sqsubseteq  \standb{s} [ \top \Rightarrow \bot ] } { \top \sqsubseteq \standball [ C \Rightarrow \bot ] }{\retB}
\qquad
\dedsr{ C \sqsubseteq  \standd{s} \bot } { \top \sqsubseteq \standball [ C \Rightarrow \bot ] }{\retC}


\subsection*{Bonus Track I: Including ABox Reasoning}

Rewrite axioms of the form $\standd{s} \alpha$ (where $\alpha$ is a concept or role assertion) into $\sp \prec \st$ and $\standb{s'} \alpha$, where $\sp$ is a fresh standpoint symbol.

Then, we rewrite every concept assertion of the form
$\standb{s} [ A(a) ]$ into $\{ a \} \sqsubseteq \standb{s} [\top \Rightarrow A] $. Role assertions are left untouched.
So we obtain a new type of normal form axiom: $\standb{s}	[	r(a,b) ]$.
\medskip

Also, for every concept name $B$, every ABox individual $a$ and every standpoint symbol $\st$, we introduce a fresh concept name $P_{\mathsf{s},a,B}$ as well as a fresh standpoint symbol denoted $\mathsf{s}[a,B]$ and add the following background axioms

\begin{align*}
	\mathsf{s}[a,B]    & \prec \mathsf{s}                                           \\
	\{a\}              & \sqsubseteq \standb{s} [ B \Rightarrow P_{\mathsf{s},a,B}] \\
	P_{\mathsf{s},a,B} & \sqsubseteq {\standb{s}}_{[a,B]} [ \top \Rightarrow B ]    \\
\end{align*}


\paragraph{Additional Deduction Rules}{$\left.\right.$}
\\

\dedsr{\top \sqsubseteq \standb{s} [B \Rightarrow C]} {\{a\} \sqsubseteq \standb{s} [B \Rightarrow C]}{\abAA}


\dedsr{\standb{s'}[R(a,b)] \quad \st \preceq \sp } {\standb{s}[R(a,b)]}{\abA}

\medskip

\dedsr{ \standb{s} [ R(a,b) ] \quad \standb{s} [ R \sqsubseteq R' ]  } { \standb{s} [ R'(a,b) ]  }{\abB}

\medskip

\dedsr{ \standb{s} [ R_1(a,b) ] \quad \standb{s} [ R_2(b,c) ] \quad \standb{s}	[ R_1 \circ R_2  \sqsubseteq R' ]  } { \standb{s} [ R'(a,c) ]  }{\abC}

\bigskip

Inference involving existential quantifiers


\medskip

\dedsr{ \standb{s} [ R(a,b) ] \quad \{b\} \sqsubseteq \standb{s}[\top \Rightarrow B] \quad \standb{s}[\exists R.B \sqsubseteq A]  } {\{a\} \sqsubseteq \standb{s}[\top \Rightarrow A] }{\abeA}

\medskip

\dedsr{ \standb{s} [ R_1(a,b) ] \quad \{b\} \sqsubseteq \standb{s}[\top \Rightarrow B] \quad \standb{s}[B \sqsubseteq \exists R_2.C ] \quad \standb{s}	[ R_1 \circ R_2  \sqsubseteq R ]  \quad \standb{s} [ R \sqsubseteq R' ] \quad \standb{s}[\exists R'.C \sqsubseteq A]  } {\{a\} \sqsubseteq \standb{s}[\top \Rightarrow A] }{tha}

\medskip

``Retraction'' of $\bot$ inference

\bigskip

\dedsr{ \{a\} \sqsubseteq \standb{s}[\top \Rightarrow \bot]  } { \top \sqsubseteq \standball[\top \Rightarrow \bot]   }{\abr}


\subsection*{Bonus Track II: Including Self Loops}

We extend the normal form by allowing concept expression $\exists R.\mathsf{Self}$ everywhere where concept names are allowed. All previous deduction rules are generalized accordingly.

We introduce the following deduction rules:

\bigskip

Interaction with other TBox statements

\medskip

\dedsr{\standb{s}[R \sqsubseteq R']} {\top \sqsubseteq \standb{s}[\exists R.\mathsf{Self} \Rightarrow \exists R'.\mathsf{Self}]}{\selfA}
\qquad
\dedsr{\standb{s} [ R_1 \circ R_2  \sqsubseteq R' ]}{\standb{s} [\exists R_1.\mathsf{Self} \sqcap \exists R_2.\mathsf{Self} \sqsubseteq \exists R'.\mathsf{Self}]}{\selfB}
\qquad
\color{red}
\dedsr{} {\standball [\exists R.\mathsf{Self} \sqcap D \sqsubseteq \exists R.D]}{\axA}

Doesn't work, not in (extended) normal form. Replacement below:\\
\color{teal}
\dedsr{\top \sqsubseteq \standbs [C \Rightarrow \exists R.\mathsf{Self}] } {\standbs [C \sqsubseteq \exists R.C]}{\axA}
\color{black}


\medskip

\dedsr{\standb{s}[B \sqsubseteq \exists R_1.D] \quad \standb{s}[D \sqsubseteq \exists R_2.\mathsf{Self}] \quad \standb{s} [ R_1 \circ R_2  \sqsubseteq R' ]}{\standb{s} [B \sqsubseteq \exists R'.D]}{\selfC}

\medskip

\dedsr{\standb{s}[B \sqsubseteq \exists R_1.\mathsf{Self}] \quad \standb{s}[B \sqsubseteq \exists R_2.D] \quad \standb{s} [ R_1 \circ R_2  \sqsubseteq R' ]}{\standb{s} [B \sqsubseteq \exists R'.D]}{\selfD}

\bigskip

Interaction with ABox statements

\medskip

\dedsr{ \standb{s} [ R(a,a) ] } {\{a\} \sqsubseteq \standb{s}[\top \Rightarrow \exists R.\mathsf{Self}]}{\selfE}
\qquad
\dedsr{ \{a\} \sqsubseteq \standb{s}[\top \Rightarrow \exists R.\mathsf{Self}] } {\standb{s} [ R(a,a) ]}{\selfF}


==> sections/conclusion.tex <==
In this paper we introduced Standpoint $\EL$, a new, lightweight member of the emerging family of standpoint logics. We described the new modelling and reasoning capabilities it brings to large-scale ontology management
and established a \textsc{PTime} (and thus worst-case optimal) tableau-based decision procedure for standard reasoning tasks. We also demonstrated that certain extensions of $\SEL$, which would be desirable from a expressivity point of view, inevitably come with a loss of tractability (sometimes under the assumption $\textsc{P} \neq \textsc{NP}$).

Yet several modelling features can be accommodated into $\SEL$ without endangering tractability.
For instance, from a usability perspective, it would seem very advantageous if not just single axioms, but whole axiom sets (up to whole knowledge bases) could be preceded by standpoint modalities. By definition, an axiom of the type $\standbs\kb$ can be equivalently rewritten into the axiom set $\{\standbs\phi \mid \phi \in \kb\}$. While something alike is not immediately possible for axioms of the type $\standds\kb$, our normalization rule for diamond-preceded axioms can be lifted and thus $\standds\kb$ can be rewritten to $\standb{s'}\kb$ (and further to $\{\standb{s'}\phi \mid \phi \in \kb\}$) upon introducing a fresh standpoint name $\sp$ and asserting $\sp \preceq \st$. Thus standpoint-modality-annotated knowledge bases come essentially for free in $\SEL$. In fact, we already made use of this modelling feature in Axiom~\ref{formula:instance-patient1} and Axiom~\ref{formula:instance-tumour} of our initial example.

Moreover, we are confident that, as opposed to nominal concepts, other modelling features of OWL~2~EL can be added to $\SEL$ without harming tractability. These include complex role inclusions (also called role-chain axioms) such as $\pred{FindingSite} \circ \pred{PartOf} \sqsubseteq \pred{FindingSite}$, and the self-concept as in $ \pred{ApoptoticCell} \sqsubseteq \exists \pred{Destroys}.\mathsf{Self}$. It also seems plausible that the sharpening statements can be extended to incorporate intersection and disjointness of standpoints.

Beyond exploring the tractability boundaries, next endeavours include to investigate feasible strategies for developing a $\SEL$ reasoner. Options include
\begin{itemize}
    \item to implement our tableau algorithm from scratch or by modifying existing open-source tableaux systems,
    \item to design a deduction calculus over normalised axioms that can be translated into a datalog program, akin to the approach of \citeauthor{Krotzsch10OWLELreasoning} [\citeyear{Krotzsch10OWLELreasoning}], then utilizing a state-of-the-art datalog engine like VLog \cite{vlog16}, or
    \item to find a reduction to reasoning in standpoint-free (\textsc{PTime} extensions of) $\EL$ that is supported by existing reasoners (such as ELK \cite{KazakovKS14} or Snorocket \cite{Metke-JimenezL13}).
\end{itemize}
With one or several reasoners in place, appropriate experiments will be designed and conducted to assess practical feasibility and scalability.

Beyond the $\EL$ family, further popular and computationally lightweight formalisms exist, such as the tractable profiles OWL~2~RL and OWL~2~QL \cite{owl2-profiles}. It would be interesting to investigate options to extend these by standpoint reasoning without sacrificing tractability. More generally, we intend to research the effect of adding standpoints to KR languages -- light- or heavyweight -- in terms of computational properties and expressivity as well as avenues for implementing efficient reasoners for them.
%-Easy extensions that add paragraphing such 
% - as diamonds in front of full ABox

%Future work:
%- Standpoint conjunction and disjointness in axiom statements.
%- Role chain axioms.
%- Implementations and optimisation, hint at complexity optimal deduction calculus. 



==> sections/intractable-extensions.tex <==
While the shown tractability of reasoning in $\SEL$ is good news, one might ask if one could include more modelling features or relax certain side conditions and still preserve tractability.
This section shows that tractability can be easily lost (at least under standard complexity-theoretic assumptions).

\subsubsection{Empty standpoints}
While it may make sense on a philosophical level, one might wonder whether the constraint that $\sigma(\st)$ needs to be nonempty for every \mbox{$\st \in \SC$} has an impact on tractability.
In fact, dropping this constraint, obtaining a logic $\SEL^\emptyset$ with the same syntax but modified semantics, would increase expressivity (standpoint non-emptiness could still be enforced in $\SEL^{\smash\emptyset}$ by asserting \mbox{$\top \sqsubseteq \standds\! \top$} for every \mbox{$\st\in\SC$}).
However, satisfiability in $\SEL^{\smash\emptyset}$ turns out to be \NP-hard, even when disallowing usage of concept and role names entirely.
The key insight that both $\standd{s}\! \top$ and its negation $\standb{s} \bot$ can be expressed as $\SEL^{\smash\emptyset}$ concepts gives rise to the following reduction from 3SAT:
Assume an instance \mbox{$\phi= \bigvee\!\clause_1 \land \ldots \land \bigvee\!\clause_n$} of 3SAT containing $n$ clauses (i.e., disjunctions of literals) $\bigvee\!\clause_j$  over the propositional variables \mbox{$P = \set{ p_1,\ldots, p_k }$}.
We note that $\phi$ is equivalent to \mbox{$(\bigwedge\!\overline{\clause}_1 \to \mathbf{false}) \wedge \ldots \wedge  (\bigwedge \!\overline{\clause}_k \to \mathbf{false})$}, where $\overline{\clause}_j$ is obtained from ${\clause}_j$ by replacing every literal by its negated version.
%
Let now $\{\st_1,\ldots,\st_k\}$ be a set of standpoint names and, for any literal $\ell$ over $P$, define
%
\begin{linenomath*}
    $$
        L_\ell = \begin{cases}
            \standd{s_i}\! \top & \text{ if } \ell = p_i,      \\
            \standb{s_i} \bot   & \text{ if } \ell = \neg p_i. \\
        \end{cases}
    $$
\end{linenomath*}
%
Then, $\phi$ is satisfiable iff the following $\SEL^\emptyset$ knowledge base is:
%
\begin{linenomath*}
    $$
        \KB_\phi = \big\{  L_{\ell} \sqcap L_{\ell'} \sqcap L_{\ell''} \sqsubseteq \bot  \mid  \{\ell,\ell',\ell''\} =  \overline{\clause}_j, 1 \leq j \leq n \big\}.
    $$
\end{linenomath*}
%

\subsubsection{Rigid roles}
$\SEL$ allows to globally enforce rigidity of specific concepts through axioms of the shape \mbox{$A \sqsubseteq \standball A$}.
(This is in contrast to e.g.\ $\mathbf{K}_n\mathcal{ALC}$, where rigidity of concepts can only be expressed \emph{relative} to a given formula.)
In a similar manner, rigidity of roles (i.e., the interpretation of certain distinguished roles being the same throughout all precisifications) would represent a desirable modelling feature.
Other modal extensions of DLs have easily been shown to even become undecidable when this feature is permitted, but as $\SEL$ uses a much simplified semantics on the modal dimension, these results do not carry over to $\SEL$.
Yet, we will show that just the presence of \emph{one} distinguished rigid role $\dot{R}$ causes $\SEL$ to become intractable as satisfiability turns \coNP-hard.
To demonstrate this, we reduce 3SAT to KB unsatisfiability.
\begin{shortonly}
    As above, assume an instance $\phi= \bigvee\!\clause_1 \land \ldots \land \bigvee\!\clause_n$ of 3SAT over propositional variables \mbox{$P = \set{ p_1,\ldots, p_k }$}.
    Then $\phi$ is satisfiable iff the following $\SEL$ TBox is unsatisfiable (with all axioms instantiated for $1 \leq i \leq k$):
    \begin{linenomath*}
        $$
            \begin{array}{@{}r@{\ }l@{}r@{\ }l}
                \top    & \sqsubseteq \exists T. L_0                                             & L_k                                                   & \sqsubseteq \standdall\mathit{S}             \\
                L_{i-1} & \sqsubseteq \exists \dot{R}.\standball(L_{i} \sqcap T_{p_i} )          & \exists \dot{R}.(T_{p_i} \sqcap \mathit{S})           & \sqsubseteq (T_{p_i} \sqcap \mathit{S})      \\
                L_{i-1} & \sqsubseteq \exists \dot{R}.\standball (L_{i} \sqcap T_{\neg p_i})     & \exists \dot{R}.(T_{\neg p_i} \sqcap \mathit{S})      & \sqsubseteq (T_{\neg p_i} \sqcap \mathit{S}) \\
                T_\ell  & \sqsubseteq T_{\clause_j} \text{\ \ for all } \ell \in \clause_j \quad & T_{\clause_1} \! \sqcap \ldots \sqcap T_{\clause_n}\! & \sqsubseteq \bot
            \end{array}
        $$
    \end{linenomath*}
\end{shortonly}
\begin{supplementary}

\end{supplementary}


\subsubsection{Nominal Concepts}
\newcommand{\ELO}{\mathcal{E\hspace{-1pt}LO}}
\newcommand{\SELO}{\mathbb{S}_\ELO}
Nominal concepts are a modelling feature widely used in ontology languages.
For an individual $o$, the nominal concept $\{o\}$ refers to the singleton set $\{o^\mathcal{I}\}$.
Let $\ELO$ denote $\EL$ extended by nominal concepts.
Several formalisms subsuming $\ELO$, including OWL~2~EL, are known to allow for tractable reasoning \cite{Baader05ELenvelope,Krotzsch10OWLELreasoning}.
However, in the presence of standpoints, nominals prove to be detrimental for the reasoning complexity: satisfiability of $\SELO$ TBoxes using just one nominal concept $\{o\}$ turns out to be \ExpTime-hard and thus definitely harder than for $\SEL$. This can be shown by a \PTime reduction of satisfiability for Horn-$\mathcal{ALC}$ TBoxes (which is known to be \ExpTime-complete \cite{Krotzsch13HornDLs}) to satisfiability of $\SELO$ TBoxes with just one standpoint (the global one) and one nominal concept $\{o\}$.
%
To this end, recall that any Horn-$\mathcal{ALC}$ TBox can be normalised in \PTime to consist of only axioms of the following shapes:
%
\begin{linenomath*}
    $$
        A \sqsubseteq B \quad\! A \sqcap B \sqsubseteq C \quad\! \exists R.A \sqsubseteq B \quad\! A \sqsubseteq \exists R.B \quad\! A \sqsubseteq \forall R.B
    $$
\end{linenomath*}
%
where $A$ and $B$ can be concept names, $\top$, or $\bot$.
From a normalised Horn-$\mathcal{ALC}$ TBox $\mathcal{T}$, we obtain the target $\SELO$ TBox $\mathcal{T}'$ by
(i) declaring every original concept name as rigid via the axiom $A \sqsubseteq \standball A$ as well as
(ii) replacing every axiom of the shape $A \sqsubseteq \exists R.B$ by the axiom
\begin{linenomath*}
    $$A \sqsubseteq \standdall ((\exists \mathit{Src}.\{o\}) \sqcap (\exists R.(B \sqcap \exists \mathit{Tgt}.\{o\})))$$
\end{linenomath*}
(introducing two fresh role names $\mathit{Src}$ and $\mathit{Tgt}$), and replacing every axiom of the shape $A \sqsubseteq \forall r.B$ by the two axioms
\begin{linenomath*}
    $$A \sqcap \exists R.\top \sqsubseteq (\exists \mathit{Src}.(\{o\} \sqcap \tilde{B})) \quad\text{and}\quad \exists \mathit{Tgt}.\tilde{B} \sqsubseteq B,$$
\end{linenomath*}
introducing a copy $\tilde{A}$ for every original concept name $A$.
%
%$$
%\begin{array}{r@{\ }lrr@{\ }l}
%	A           & \sqsubseteq B           & \Longrightarrow &  A           & \sqsubseteq B  \\
%	A \sqcap B  & \sqsubseteq C           & \Longrightarrow &  A \sqcap B  & \sqsubseteq C \\
%	A           & \sqsubseteq \exists r.B & \Longrightarrow &  A           & \sqsubseteq \standdall ((\exists src.\{o\}) \sqcap (\exists r.(B \sqcap \exists tgt.\{o\})))  \\
%	\exists r.A & \sqsubseteq B           & \Longrightarrow & \exists r.A  & \sqsubseteq B \\
%	A           & \sqsubseteq \forall r.B & \Longrightarrow & A \sqcap \exists r.\top & \sqsubseteq (\exists src.(\{o\} \sqcap \tilde{B})) \qquad   \exists tgt.\tilde{B} \sqsubseteq B\\
%\end{array}
%$$
With this polytime translation, satisfiability of the Horn-$\mathcal{ALC}$ TBox $\mathcal{T}$ and the $\SELO$ TBox $\mathcal{T}'$ coincide.

\begin{supplementary}
    \begin{proposition}
        $\mathcal{T}$ and $\mathcal{T}'$ are equisatisfiable.
    \end{proposition}
    \begin{proof}
        We show equisatisfiability of $\mathcal{T}$ and $\mathcal{T}'$ by providing constructions to obtain a model of $\mathcal{T}$ from a model of $\mathcal{T}'$ and vice versa.
        Let $\mathcal{I}=(\Dom,\cdot^\mathcal{I})$ be a model of $\mathcal{T}$. Then we construct a model
        $\dlstruct= \tuple{\Dom, \Precs, \sigma, \gamma}$ of $\mathcal{T}'$ as follows:
        \begin{itemize}
            \item $\Precs = \Roles \times \Dom \times \Dom$ with $\sigma(*) = \Precs$,
            \item pick one arbitrary but fixed $\delta_o \in \Dom$ and let $o^{\gamma(\pi)}=\delta_o$ for all $\pi \in \Precs$,
            \item $A^{\gamma(\pi)}=A^\mathcal{I}$ for all $\pi \in \Precs$, whereas
                  $\tilde{A}^{\gamma((r,\delta_1,\delta_2))}= \{ \delta_o \mid \delta_2 \in A^\mathcal{I}\}$ for $A \in \Concepts$,
            \item $r^{\gamma((r,\delta_1,\delta_2))}=\{(\delta_1,\delta_2)\} \cap r^\mathcal{I}$, while
                  $src^{\gamma((r,\delta_1,\delta_2))}=\{(\delta_1,\delta_o)\}$ and
                  $tgt^{\gamma((r,\delta_1,\delta_2))}=\{(\delta_2,\delta_o)\}$.
        \end{itemize}

        \medskip

        For the other direction, let $\dlstruct= \tuple{\Dom, \Precs, \sigma, \gamma}$ be a model of $\mathcal{T}'$. Then we construct a model $\mathcal{I}=(\Dom,\cdot^\mathcal{I})$ of $\mathcal{T}$ as follows:
        \begin{itemize}
            \item $A^\mathcal{I} = A^{\gamma(\pi)}$ for any $\pi \in \Precs$ (the choice is irrelevant because all $A$ are rigid)
            \item $r^\mathcal{I} = \bigcup_{\pi \in \Precs}\{(\delta_1,\delta_2) \in r^{\gamma(\pi)} \mid (\delta_1,o^{\gamma(\pi)}) \in  src^{\gamma(\pi)},\ (\delta_2,o^{\gamma(\pi)}) \in tgt^{\gamma(\pi)}\}$
        \end{itemize}
    \end{proof}
\end{supplementary}




==> sections/proofs-section-4.tex <==
\newcommand{\SELO}{\SEL ?}
\begin{theorem}
    Satisfiability of $\SEL$ TBoxes with $*$ as the only occurring standpoint name and one distinguished rigid role $\dot{R}$ is \coNP-hard.
    \begin{proof}
        We reduce the \NP-hard problem SAT to TBox unsatisfiability.
        Assume an instance $\phi=\clause_1 \land \ldots \land \clause_n$ of SAT containing $n$ clauses $\clause_j$ (disjunctions of literals) over the propositional variables \mbox{$P = \set{ p_1,\ldots, p_k }$}.

        We construct the following $\SELO$ TBox $\T_\phi$ (of polynomial size):
        \begin{align}
            \top                                                  & \sqsubseteq \exists U. L_0                                                                                                                    \label{lstart}                                                                                    \\
            L_{i-1}                                               & \sqsubseteq \exists \dot{R}.(T_{p_i} \sqcap L_{i} ) \sqcap \exists \dot{R}. (T_{\neg p_i} \sqcap L_{i})                                                      & \text{ for all } 1\leq i\leq k      \label{lnext}                                \\
            L_{i} \sqcap T_{p_i}                                  & \sqsubseteq \standball ( L_{i} \sqcap T_{p_i} )                                                                                                              & \text{ for all } 1\leq i\leq k                                     \label{ltrue} \\
            L_{i} \sqcap T_{\neg p_i}                             & \sqsubseteq \standball ( L_{i} \sqcap T_{\neg p_i} )                                                                                                         & \text{ for all } 1\leq i\leq k      \label{lfalse}                               \\
            L_k                                                   & \sqsubseteq \standdall\!\mathit{Select}                                                                        \label{sstart}                                                                                                                   \\
            \exists \dot{R}.(T_{p_i} \sqcap \mathit{Select})      & \sqsubseteq (T_{p_i} \sqcap \mathit{Select})                                                                                                                 & \text{ for all } 1\leq i\leq k                       \label{strue}               \\
            \exists \dot{R}.(T_{\neg p_i} \sqcap \mathit{Select}) & \sqsubseteq (T_{\neg p_i} \sqcap \mathit{Select})                                                                                                            & \text{ for all } 1\leq i\leq k  \label{sfalse}                                   \\
            T_\ell                                                & \sqsubseteq T_{\clause_j}                                                                                                                                    & \text{ for all } \ell \in \clause_j \label{clause}                               \\
            T_{\clause_1} \sqcap \ldots \sqcap T_{\clause_n}      & \sqsubseteq \bot  \label{disjoint}
        \end{align}
        We conclude the proof by showing that $\phi$ is satisfiable iff $\T_\phi$ is unsatisfiable.
        \begin{description}
            \item[\normalfont``if'':]
                We show the contrapositive.
                Let $\phi$ be unsatisfiable.
                We construct a model \mbox{$\dlstruct= \tuple{\Dom, \Precs, \sigma, \gamma}$} for $\T_\phi$ as follows.
                \begin{align*}
                    \Dom   & = \set{ w\in\set{0,1}^* \guard \abs{w}\leq k } \\
                    \Precs & = 2^P
                \end{align*}
                That is, the interpretation domain contains all words $w$ over $\set{0,1}$ of length at most $k$ (including the empty word $\nil$).
                Roughly, each $w$ encodes a partial interpretation of $P$ where $w_i$, the $i$-th symbol in $w$, encodes whether $p_i$ is true ($w_i=1$) or false ($w_i=0$) or undefined ($\abs{w}<i$).

                Finally, for each $Q\subseteq P$, the DL interpretation $\gamma(Q)=\tuple{\Dom,\intf}$ is given by
                \begin{align*}
                    \interprets{U}               & = \Dom\times\set{ \nil }                                                                           \\
                    \interprets{\dot{R}}         & = \set{ \tuple{w,w0}, \tuple{w,w1} \guard w,w0,w1\in\Dom }                                         \\
                    \interprets{L_i}             & = \set{ w\in\Dom \guard \abs{w}=i }                                                                \\
                    \interprets{T_{p_i}}         & = \set{ w\in\Dom \guard w_i=1 } \cup \set{ w\in\Dom \guard w\in\prefixes(w^Q), \abs{w}<i, w^Q_i=1} \\
                    \interprets{T_{\neg p_i}}    & = \set{ w\in\Dom \guard w_i=0 } \cup \set{ w\in\Dom \guard w\in\prefixes(w^Q), \abs{w}<i, w^Q_i=0} \\
                    \interprets{\mathit{Select}} & = \prefixes(w^Q)                                                                                   \\
                    \interprets{T_{\clause_j}}   & = \bigcup_{\ell\in\clause_j}\interprets{T_{\ell}}
                \end{align*}
                Where the word $w^Q$ of length $k$ encodes the valuation $Q$ via
                \[
                    w^Q_i               = \begin{cases}
                        0 & \text{ if } p_i\notin Q \\
                        1 & \text{ otherwise}
                    \end{cases}
                \]
                and $\prefixes(w)=\set{v\in\set{0,1}^* \guard \exists u\in\set{0,1}^*: w=vu}$ denotes the set of all prefixes of $w\in\set{0,1}^*$.
                %Observe that $Q\models p_i$ iff $w^Q\in T_{p_i}$, and $Q\not\models p_i$ iff $w^Q\in T_{\neg p_i}$.

                We now show that $\dlstruct\models\T_\phi$.
                Unless declared otherwise, assume that $\struct=\gamma(Q)$ is for an arbitrary $Q\subseteq P$.

                We note that the interpretations of the $L_i$ ($0\leq i\leq k$) and $T_{\clause_j}$ ($1\leq j\leq n$) is the same across precisifications, and for $T_{p_i}$ and $T_{\neg p_i}$ their extensions agree on all words of length at least $i$.
                \begin{itemize}
                    \item (\ref{lstart}): By definition.
                    \item (\ref{lnext}): Let $w\in\interprets{L_{i-1}}$.
                          Then $\abs{w}=i-1$.
                          In particular, since $i-1<k$, we have $w0,w1\in\Dom$ and thus $\tuple{w,w0},\tuple{w,w1}\in\interprets{\dot{R}}$.
                          Clearly, $\abs{w0}=\abs{w1}=i$ whence $w0,w1\in\interprets{L_i}$.
                          Furthermore, $(w0)_i=0$ whence $w0\in T_{\neg p_i}$;
                          likewise $(w1)_i=1$ and $w1\in T_{p_i}$.
                    \item (\ref{ltrue}): Let $w\in\interprets{L_i}\cap\interprets{T_{p_i}}$.
                          Then $\abs{w}=i$ and $w_i=1$ by definition.
                          Thus by agreement across precisifications, for any $Q\subseteq P$ we get $w\in(L_i\dland T_{p_i})^{\gamma(Q)}$, whence $w\in \bigcap_{Q\subseteq P} (L_i\dland T_{p_i})^{\gamma(Q)}$.
                    \item (\ref{lfalse}): Symmetric.
                    \item (\ref{sstart}): Let $w\in\interprets{L_k}$.
                          Then $\abs{w}=k$ and there is a $Q\subseteq P$ such that $w^Q=w$.
                          Since $w=w^Q\in\prefixes(w^Q)$ by definition, for $\gamma(Q)$ we thus have $w\in (\mathit{Select})^{\gamma(Q)}$.
                    \item (\ref{strue}): Let $\tuple{v,w}\in\interprets{\dot{R}}$ such that $w\in\interprets{T_{p_i}}\cap\interprets{\mathit{Select}}$.
                          Then $w\in\prefixes(w^Q)$, and either
                          (a) $\abs{w}=i$ and $w_i=1$, or
                          (b) $\abs{w}<i$ and $w^Q_i=1$.
                          By definition of $\interprets{\dot{R}}$ we have $v\in\prefixes(w)\subseteq\prefixes(w^Q)$, whence $v\in\interprets{\mathit{Select}}$.
                          In particular, $\abs{v}=i-1<i$ and in any case we have $w^Q_i=1$, thus $v\in\interprets{T_{p_i}}$.
                    \item (\ref{sfalse}): Symmetric.
                    \item (\ref{clause}): By definition.
                    \item (\ref{disjoint}): By contradiction:
                          Assume that there is a $Q\subseteq P$ such that for $\struct=\gamma(Q)$, there is some $w\in\interprets{T_{\clause_1}}\cap\ldots\cap\interprets{T_{\clause_n}}$.
                          Then by definition, for each $1\leq j\leq n$ there is an $\ell_j\in\clause_j$ such that $w\in\interprets{T_{\ell_j}}$.
                          Define $R_w = \set{ p\in P \guard w\in \interprets{T_{p}} } \cup \set{ \neg p \guard p\in P, w\in\interprets{T_{\neg p}}}$.
                          $R_w$ is consistent because for all $1\leq i\leq k$, we have $\interprets{T_{p_i}}\cap\interprets{T_{\neg p_i}}=\emptyset$.
                          We show $R_w\cap P\models\phi$ to obtain the desired contradiction with unsatisfiability of $\phi$.
                          Consider $\clause_j$.
                          We have $\ell_j\in\clause_j$ as above with $w\in\interprets{T_{\ell_j}}$, whence by definition $\ell_j\in R_w$.
                          Consequently, $R_w\cap P\models\ell_j$.
                          Since $\clause_j$ was chosen arbitrarily, we get $R_w\cap P\models\phi$.
                \end{itemize}
            \item[\normalfont``only if'':]
                Let $\phi$ be satisfiable.
                Then there is a $Q\subseteq P$ such that $Q\models\phi$.
                We show by contradiction that $\T_\phi$ is unsatisfiable.
                Assume that there is a Standpoint DL structure $\dlstruct=\tuple{\Dom,\Precs,\sigma,\gamma}$ such that $\dlstruct\models\T_\phi$.
                By $\dlstruct\models (\ref{lstart}) \land (\ref{lnext})$, in every $\pr\in\Precs$, $\dot{R}$ contains a full binary tree of depth $k$ where in each layer $i$, the nodes (individuals $\de_i\in\Dom$) are marked with $L_i$, and one of $T_{p_i}$ and $T_{\neg p_i}$, respectively.
                Due to the rigid role $\dot{R}$ being used and rigidity of $L_i\dland T_{(\neg)p_i}$ being enforced by (\ref{ltrue}) and (\ref{lfalse}), this part of the interpretation is “the same” across precisifications.
                Employing $\dlstruct\models (\ref{sstart})$, we now consider $\pr\in\Precs$ and the sequence
                $\de_0,\ldots,\de_k\in\Dom$ with $\de_0\in\interpretgp{L_0}$,
                $\tuple{\de_{i-1},\de_i}\in\interpretgp{\dot{R}}$ for all $1\leq i\leq k$,
                $\de_i\in\interpretgp{L_i}\cap\interpretgp{\mathit{Select}}$ for all $1\leq i\leq k$ such that for all $p_i\in P$:
                \begin{itemize}
                    \item $\de_i\in\interpretgp{T_{p_i}}$ whenever $p_i\in Q$,
                    \item $\de_i\in\interpretgp{T_{\neg p_i}}$ whenever $p_i\notin Q$.
                \end{itemize}
                Since $\dlstruct\models (\ref{lnext}) \land (\ref{strue}) \land (\ref{sfalse})$, it follows that for all $p\in P$:
                \begin{itemize}
                    \item $\de_1\in\interpretgp{T_{p}}$ whenever $p\in Q$,
                    \item $\de_1\in\interpretgp{T_{\neg p}}$ whenever $p\notin Q$.
                \end{itemize}
                Now since $Q\models\phi$, we get that $Q\models\clause_j$ for all $1\leq j\leq k$;
                that is, for every $\clause_j$ there is a literal $\ell_j\in\clause_j$ such that $Q\models\ell_j$.
                Now $Q\models\ell_j$ iff $\de_1\in\interpretgp{T_{\ell_j}}$ by the above.
                Thus, for every $\clause_j$ there is $\ell_j\in\clause_j$ such that $\de_1\in\interpretgp{T_{\ell_j}}$.
                Thus $\de_1\in T_{\clause_j}$ by $\dlstruct\models (\ref{clause})$.
                But then, since $\clause_j$ was chosen arbitrarily, we get $\de_1 \in \interpretgp{(T_{\clause_1}\dland\ldots\dland T_{\clause_n})}$ in contradiction to $\dlstruct\models (\ref{disjoint})$.
        \end{description}
    \end{proof}
\end{theorem}

\begin{definition}
    From a normalised Horn-$\mathcal{ALC}$ TBox $\mathcal{T}$, we obtain the target $\SELO$ TBox $\SELO(\mathcal{T})$ by
    \begin{itemize}[leftmargin=0.7cm]
        \item[(i)] declaring every original concept name as rigid via the axiom $A \sqsubseteq \standball A$ as well as
        \item[(ii)] replacing every axiom of the shape $A \sqsubseteq \exists R.B$ by the axiom
            \begin{linenomath*}
                $$A \sqsubseteq \standdall ((\exists \mathit{Src}.\{o\}) \sqcap (\exists R.(B \sqcap \exists \mathit{Tgt}.\{o\})))$$
            \end{linenomath*}
            (introducing two fresh role names $\mathit{Src}$ and $\mathit{Tgt}$), and replacing every axiom of the shape $A \sqsubseteq \forall r.B$ by the two axioms
            \begin{linenomath*}
                $$A \sqcap \exists R.\top \sqsubseteq (\exists \mathit{Src}.(\{o\} \sqcap \tilde{B})) \quad\text{and}\quad \exists \mathit{Tgt}.\tilde{B} \sqsubseteq B,$$
            \end{linenomath*}
            introducing a copy $\tilde{A}$ for every original concept name $A$.
    \end{itemize}
\end{definition}


\begin{theorem}
    Let $\mathcal{T}$ be a normalised Horn-$\mathcal{ALC}$ TBox. Then, $\mathcal{T}$ and $\SELO(\mathcal{T})$ are equisatisfiable.
\end{theorem}
\begin{proof}
    We show equisatisfiability of $\mathcal{T}$ and $\SELO(\mathcal{T})$ by providing constructions to obtain a model of $\mathcal{T}$ from a model of $\mathcal{T}'$ and vice versa.
    Let $\mathcal{I}=(\Dom,\cdot^\mathcal{I})$ be a model of $\mathcal{T}$. Then we construct a model
    $\dlstruct= \tuple{\Dom, \Precs, \sigma, \gamma}$ of $\SELO(\mathcal{T})$ as follows:
    \begin{itemize}
        \item $\Precs = \Roles \times \Dom \times \Dom$ with $\sigma(*) = \Precs$,
        \item pick one arbitrary but fixed $\delta_o \in \Dom$ and let $o^{\gamma(\pi)}=\delta_o$ for all $\pi \in \Precs$,
        \item $A^{\gamma(\pi)}=A^\mathcal{I}$ for all $\pi \in \Precs$, whereas
              $\tilde{A}^{\gamma((r,\delta_1,\delta_2))}= \{ \delta_o \mid \delta_2 \in A^\mathcal{I}\}$ for $A \in \Concepts$,
        \item $R^{\gamma((r,\delta_1,\delta_2))}=\{(\delta_1,\delta_2)\} \cap R^\mathcal{I}$, while
              $Src^{\gamma((r,\delta_1,\delta_2))}=\{(\delta_1,\delta_o)\}$ and
              $Tgt^{\gamma((r,\delta_1,\delta_2))}=\{(\delta_2,\delta_o)\}$.
    \end{itemize}

    \medskip

    For the other direction, let $\dlstruct= \tuple{\Dom, \Precs, \sigma, \gamma}$ be a model of $\SELO(\mathcal{T})$. Then we construct a model $\mathcal{I}=(\Dom,\cdot^\mathcal{I})$ of $\mathcal{T}$ as follows:
    \begin{itemize}
        \item $A^\mathcal{I} = A^{\gamma(\pi)}$ for any $\pi \in \Precs$ (the choice is irrelevant because all $A$ are rigid)
        \item $R^\mathcal{I} = \bigcup_{\pi \in \Precs}\{(\delta_1,\delta_2) \in R^{\gamma(\pi)} \mid (\delta_1,o^{\gamma(\pi)}) \in  Src^{\gamma(\pi)},\ (\delta_2,o^{\gamma(\pi)}) \in Tgt^{\gamma(\pi)}\}$
    \end{itemize}
\end{proof}

